emrQA: A Large Corpus for Question Answering on Electronic Medical Records

We propose a novel methodology to generate domain-specific large-scale question answering (QA) datasets by re-purposing existing annotations for other NLP tasks. We demonstrate an instance of this methodology in generating a large-scale QA dataset for electronic medical records by leveraging existing expert annotations on clinical notes for various NLP tasks from the community shared i2b2 datasets. The resulting corpus (emrQA) has 1 million question-logical form and 400,000+ question-answer evidence pairs. We characterize the dataset and explore its learning potential by training baseline models for question to logical form and question to answer mapping.

==> tickz/hist-formulasize.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
title={Formula Size Bins},
xlabel={Formula Size},
ylabel={Frequency},
xmin=-2.05, xmax=131.05,
ymin=0, ymax=15.75,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\draw[fill=color0,draw opacity=0] (axis cs:4,0) rectangle (axis cs:8.03333333333333,7);
\draw[fill=color0,draw opacity=0] (axis cs:8.03333333333333,0) rectangle (axis cs:12.0666666666667,15);
\draw[fill=color0,draw opacity=0] (axis cs:12.0666666666667,0) rectangle (axis cs:16.1,7);
\draw[fill=color0,draw opacity=0] (axis cs:16.1,0) rectangle (axis cs:20.1333333333333,11);
\draw[fill=color0,draw opacity=0] (axis cs:20.1333333333333,0) rectangle (axis cs:24.1666666666667,7);
\draw[fill=color0,draw opacity=0] (axis cs:24.1666666666667,0) rectangle (axis cs:28.2,8);
\draw[fill=color0,draw opacity=0] (axis cs:28.2,0) rectangle (axis cs:32.2333333333333,3);
\draw[fill=color0,draw opacity=0] (axis cs:32.2333333333333,0) rectangle (axis cs:36.2666666666667,6);
\draw[fill=color0,draw opacity=0] (axis cs:36.2666666666667,0) rectangle (axis cs:40.3,3);
\draw[fill=color0,draw opacity=0] (axis cs:40.3,0) rectangle (axis cs:44.3333333333333,4);
\draw[fill=color0,draw opacity=0] (axis cs:44.3333333333333,0) rectangle (axis cs:48.3666666666667,2);
\draw[fill=color0,draw opacity=0] (axis cs:48.3666666666667,0) rectangle (axis cs:52.4,3);
\draw[fill=color0,draw opacity=0] (axis cs:52.4,0) rectangle (axis cs:56.4333333333333,3);
\draw[fill=color0,draw opacity=0] (axis cs:56.4333333333333,0) rectangle (axis cs:60.4666666666667,1);
\draw[fill=color0,draw opacity=0] (axis cs:60.4666666666667,0) rectangle (axis cs:64.5,1);
\draw[fill=color0,draw opacity=0] (axis cs:64.5,0) rectangle (axis cs:68.5333333333333,2);
\draw[fill=color0,draw opacity=0] (axis cs:68.5333333333333,0) rectangle (axis cs:72.5666666666667,2);
\draw[fill=color0,draw opacity=0] (axis cs:72.5666666666667,0) rectangle (axis cs:76.6,0);
\draw[fill=color0,draw opacity=0] (axis cs:76.6,0) rectangle (axis cs:80.6333333333333,1);
\draw[fill=color0,draw opacity=0] (axis cs:80.6333333333333,0) rectangle (axis cs:84.6666666666667,0);
\draw[fill=color0,draw opacity=0] (axis cs:84.6666666666667,0) rectangle (axis cs:88.7,1);
\draw[fill=color0,draw opacity=0] (axis cs:88.7,0) rectangle (axis cs:92.7333333333333,1);
\draw[fill=color0,draw opacity=0] (axis cs:92.7333333333333,0) rectangle (axis cs:96.7666666666667,1);
\draw[fill=color0,draw opacity=0] (axis cs:96.7666666666667,0) rectangle (axis cs:100.8,0);
\draw[fill=color0,draw opacity=0] (axis cs:100.8,0) rectangle (axis cs:104.833333333333,2);
\draw[fill=color0,draw opacity=0] (axis cs:104.833333333333,0) rectangle (axis cs:108.866666666667,0);
\draw[fill=color0,draw opacity=0] (axis cs:108.866666666667,0) rectangle (axis cs:112.9,0);
\draw[fill=color0,draw opacity=0] (axis cs:112.9,0) rectangle (axis cs:116.933333333333,1);
\draw[fill=color0,draw opacity=0] (axis cs:116.933333333333,0) rectangle (axis cs:120.966666666667,0);
\draw[fill=color0,draw opacity=0] (axis cs:120.966666666667,0) rectangle (axis cs:125,2);
\end{axis}

\end{tikzpicture}

==> tickz/pie-relations.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color7}{rgb}{0.737254901960784,0.741176470588235,0.133333333333333}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color8}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}

\begin{axis}[
xmin=-1.49436276668998, xmax=1.49025114804148,
ymin=-1.11322140836957, ymax=1.11079734744646,
tick pos=left
]
\path [fill=color0, draw opacity=0] (axis cs:1,0)
.. controls (axis cs:1,0.100452207286263) and (axis cs:0.984864031076976,0.200333437647066) .. (axis cs:0.955102493960821,0.296275591350045)
.. controls (axis cs:0.925340956844667,0.392217745053024) and (axis cs:0.881292184587856,0.483130139127178) .. (axis cs:0.824441547940362,0.56594711239629)
--(axis cs:0,0)
--(axis cs:1,0)
--cycle;

\path [fill=color1, draw opacity=0] (axis cs:0.824441547940362,0.56594711239629)
.. controls (axis cs:0.745345149498682,0.681170524159375) and (axis cs:0.642964870661683,0.778542773365584) .. (axis cs:0.523922631217077,0.85176585779108)
.. controls (axis cs:0.404880391772471,0.924988942216576) and (axis cs:0.271799281705898,0.97244939473935) .. (axis cs:0.133286939579503,0.991077490278903)
.. controls (axis cs:-0.00522540254689186,1.00970558581846) and (axis cs:-0.146116863977045,0.999090855191) .. (axis cs:-0.280274635418364,0.959919855373928)
.. controls (axis cs:-0.414432406859683,0.920748855556856) and (axis cs:-0.53890032831043,0.853884717635631) .. (axis cs:-0.645627859165002,0.763652190116689)
.. controls (axis cs:-0.752355390019574,0.673419662597748) and (axis cs:-0.838990794300198,0.561807014858566) .. (axis cs:-0.899930525069522,0.436033313002683)
.. controls (axis cs:-0.960870255838845,0.310259611146799) and (axis cs:-0.994771509078274,0.173096272608348) .. (axis cs:-0.999441563863384,0.0334149730257828)
.. controls (axis cs:-1.00411161864849,-0.106266326556782) and (axis cs:-0.97944757054808,-0.245387716506417) .. (axis cs:-0.927044681364676,-0.374950875120284)
.. controls (axis cs:-0.874641792181271,-0.504514033734151) and (axis cs:-0.795654757042226,-0.62166404308183) .. (axis cs:-0.695192429106582,-0.718823682493065)
--(axis cs:0,0)
--(axis cs:0.824441547940362,0.56594711239629)
--cycle;

\path [fill=color2, draw opacity=0] (axis cs:-0.695192429106581,-0.718823682493065)
.. controls (axis cs:-0.679174973013027,-0.734314566392669) and (axis cs:-0.662644218770554,-0.749265751061439) .. (axis cs:-0.64562785469636,-0.763652193894692)
.. controls (axis cs:-0.628611490622166,-0.778038636727944) and (axis cs:-0.611119022587968,-0.791852301009997) .. (axis cs:-0.593179749741064,-0.80507004943491)
--(axis cs:0,0)
--(axis cs:-0.695192429106581,-0.718823682493065)
--cycle;

\path [fill=color3, draw opacity=0] (axis cs:-0.593179749741064,-0.80507004943491)
.. controls (axis cs:-0.467046651899912,-0.898005564132043) and (axis cs:-0.320820392538939,-0.960010856185589) .. (axis cs:-0.166329369560993,-0.986070251463577)
.. controls (axis cs:-0.0118383465830466,-1.01212964674157) and (axis cs:0.146636358450153,-1.00152101657604) .. (axis cs:0.296275557816364,-0.955102504363067)
--(axis cs:0,0)
--(axis cs:-0.593179749741064,-0.80507004943491)
--cycle;

\path [fill=color4, draw opacity=0] (axis cs:0.296275557816364,-0.955102504363067)
.. controls (axis cs:0.328202911841007,-0.945198546850612) and (axis cs:0.359613587221914,-0.933699904784621) .. (axis cs:0.390389252697135,-0.920649896202988)
.. controls (axis cs:0.421164918172356,-0.907599887621355) and (axis cs:0.451266878806603,-0.893014920592915) .. (axis cs:0.480581733568355,-0.876949940053841)
--(axis cs:0,0)
--(axis cs:0.296275557816364,-0.955102504363067)
--cycle;

\path [fill=color5, draw opacity=0] (axis cs:0.480581733568355,-0.876949940053841)
.. controls (axis cs:0.519674567100141,-0.855526480343414) and (axis cs:0.557291161819931,-0.831512943505331) .. (axis cs:0.593179721475027,-0.805070070261471)
.. controls (axis cs:0.629068281130123,-0.778627197017611) and (axis cs:0.663148550247014,-0.749814120008947) .. (axis cs:0.695192403868657,-0.718823706901295)
--(axis cs:0,0)
--(axis cs:0.480581733568355,-0.876949940053841)
--cycle;

\path [fill=color6, draw opacity=0] (axis cs:0.695192403868657,-0.718823706901295)
.. controls (axis cs:0.751312126033,-0.664548918547343) and (axis cs:0.800883294538391,-0.603888337688352) .. (axis cs:0.842892251184842,-0.538082384856212)
.. controls (axis cs:0.884901207831293,-0.472276432024072) and (axis cs:0.919059646813812,-0.401776730865715) .. (axis cs:0.944669077803898,-0.328024897593359)
--(axis cs:0,0)
--(axis cs:0.695192403868657,-0.718823706901295)
--cycle;

\path [fill=lightgray!66.405228758169926!black, draw opacity=0] (axis cs:0.944669077803898,-0.328024897593359)
.. controls (axis cs:0.955634358479551,-0.29644631420006) and (axis cs:0.965009323080471,-0.264337758705022) .. (axis cs:0.9727586539518,-0.231820191445615)
.. controls (axis cs:0.98050798482313,-0.199302624186208) and (axis cs:0.986621938557148,-0.166416930229949) .. (axis cs:0.991077482479387,-0.13328699757411)
--(axis cs:0,0)
--(axis cs:0.944669077803898,-0.328024897593359)
--cycle;

\path [fill=color7, draw opacity=0] (axis cs:0.991077482479387,-0.13328699757411)
.. controls (axis cs:0.992562387383539,-0.12224574193092) and (axis cs:0.993862678332799,-0.111180442911099) .. (axis cs:0.994977810720474,-0.100095735043473)
.. controls (axis cs:0.996092943108149,-0.0890110271758472) and (axis cs:0.9970227612272,-0.0779084582291449) .. (axis cs:0.997766875637734,-0.0667926783421248)
--(axis cs:0,0)
--(axis cs:0.991077482479387,-0.13328699757411)
--cycle;

\path [fill=color8, draw opacity=0] (axis cs:0.997766875637734,-0.0667926783421248)
.. controls (axis cs:0.998510990048268,-0.0556768984551046) and (axis cs:0.999069296848853,-0.0445494597351107) .. (axis cs:0.999441562201348,-0.0334150227372208)
.. controls (axis cs:0.999813827553843,-0.0222805857393308) and (axis cs:0.999999999478467,-0.0111407051759998) .. (axis cs:0.999999999999999,-4.68133783078226e-08)
--(axis cs:0,0)
--(axis cs:0.997766875637734,-0.0667926783421248)
--cycle;

\node at (axis cs:1.0506127433569,0.32590315048505)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ reveals};
\node at (axis cs:-0.710190645081502,0.840017409128358)[
  scale=1.1,
  anchor= east,
  text=black,
  rotate=0.0
]{ None};
\node at (axis cs:-0.710190640165996,-0.840017413284161)[
  scale=1.1,
  anchor= east,
  text=black,
  rotate=0.0
]{ causes};
\node at (axis cs:-0.182962306517091,-1.08467727660994)[
  scale=1.1,
  anchor= east,
  text=black,
  rotate=0.0
]{ given};
\node at (axis cs:0.429428177966848,-1.01271488582329)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ improves/causes/worsens};
\node at (axis cs:0.652497693622529,-0.885577077287618)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ conducted};
\node at (axis cs:0.927181476303326,-0.591890623341833)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ reveals/conducted};
\node at (axis cs:1.07003451934698,-0.255002210590176)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ relates};
\node at (axis cs:1.09447559179252,-0.11010530854782)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ given/causes};
\node at (axis cs:1.09938571842148,-0.0367565250109428)[
  scale=1.1,
  anchor= west,
  text=black,
  rotate=0.0
]{ given/conducted};
\end{axis}

\end{tikzpicture}
